Multitask Multimodal Self-Supervised Learning for Medical Images

This thesis works to address a pivotal challenge in medical image analysis: the reliance on extensive labeled datasets, which are often limited due to the need for expert annotation and constrained by privacy and legal issues. By focusing on the development of self-supervised learning techniques and domain adaptation methods, this research aims to circumvent these limitations, presenting a novel approach to enhance the utility and efficacy of deep learning in medical imaging. Central to this thesis is the development of the Medformer, an innovative neural network architecture designed for multitask learning and deep domain adaptation. This model is adept at pre-training on diverse medical image datasets, handling varying sizes and modalities, and is equipped with a dynamic input-output adaptation mechanism. This enables efficient processing and integration of a wide range of medical image types, from 2D X-rays to complex 3D MRIs, thus mitigating the dependency on large labeled datasets. Further, the thesis explores the current state of self-supervised learning in medical imaging. It introduces novel pretext tasks that are capable of extracting meaningful information from unlabeled data, significantly advancing the model's interpretative abilities. This approach is validated through rigorous experimentation, including the use of the MedMNIST dataset, demonstrating the model's proficiency in learning generalized features applicable to various downstream tasks. In summary, this thesis contributes to the advancement of medical image analysis by offering a scalable, adaptable framework that reduces reliance on labeled data. It paves the way for more accurate, efficient diagnostic tools in healthcare, signifying a major step forward in the application of deep learning in medical imaging.

==> Preamble/preamble.tex <==
% ******************************************************************************
% ****************************** Custom Margin *********************************

% Add `custommargin' in the document class options to use this section
% Set {innerside margin / outerside margin / topmargin / bottom margin}  and
% other page dimensions
\ifsetCustomMargin
  \RequirePackage[left=37mm,right=30mm,top=35mm,bottom=30mm]{geometry}
  \setFancyHdr % To apply fancy header after geometry package is loaded
\fi

% Add spaces between paragraphs
%\setlength{\parskip}{0.5em}
% Ragged bottom avoids extra whitespaces between paragraphs
\raggedbottom
% To remove the excess top spacing for enumeration, list and description
\usepackage{enumitem}
%\setlist[enumerate,itemize,description]{topsep=0em}
\usepackage{acronym}

\usepackage{tikz}
    \usetikzlibrary{matrix,chains,positioning,decorations.pathreplacing,arrows}
    \usetikzlibrary{shapes.geometric}
    \usetikzlibrary{positioning}
    \usetikzlibrary{arrows.meta}
    \usetikzlibrary{backgrounds}
    \usetikzlibrary{external}
    \usetikzlibrary{calc}

\usepackage{minted}
\usepackage{enumitem}
% \tikzexternalize

% *****************************************************************************
% ******************* Fonts (like different typewriter fonts etc.)*************

% Add `customfont' in the document class option to use this section

\ifsetCustomFont
  % Set your custom font here and use `customfont' in options. Leave empty to
  % load computer modern font (default LaTeX font).
  %\RequirePackage{helvet}

  % For use with XeLaTeX
  %  \setmainfont[
  %    Path              = ./libertine/opentype/,
  %    Extension         = .otf,
  %    UprightFont = LinLibertine_R,
  %    BoldFont = LinLibertine_RZ, % Linux Libertine O Regular Semibold
  %    ItalicFont = LinLibertine_RI,
  %    BoldItalicFont = LinLibertine_RZI, % Linux Libertine O Regular Semibold Italic
  %  ]
  %  {libertine}
  %  % load font from system font
  %  \newfontfamily\libertinesystemfont{Linux Libertine O}
\fi

% *****************************************************************************
% **************************** Custom Packages ********************************

% ************************* Algorithms and Pseudocode **************************

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amsmath}


% ********************Captions and Hyperreferencing / URL **********************

% Captions: This makes captions of figures use a boldfaced small font.
%\RequirePackage[small,bf]{caption}

\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty


% *************************** Graphics and figures *****************************

%\usepackage{rotating}
%\usepackage{wrapfig}

% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
\usepackage{subcaption}

% ********************************** Tables ************************************
\usepackage{booktabs} % For professional looking tables
\usepackage{multirow}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}


% *********************************** SI Units *********************************
\usepackage{siunitx} % use this package module for SI units


% ******************************* Line Spacing *********************************

% Choose linespacing as appropriate. Default is one-half line spacing as per the
% University guidelines

% \doublespacing
% \onehalfspacing
% \singlespacing


% ************************ Formatting / Footnote *******************************

% Don't break enumeration (etc.) across pages in an ugly manner (default 10000)
%\clubpenalty=500
%\widowpenalty=500

%\usepackage[perpage]{footmisc} %Range of footnote options


% *****************************************************************************
% *************************** Bibliography  and References ********************

%\usepackage{cleveref} %Referencing without need to explicitly state fig /table

% Add `custombib' in the document class option to use this section
\ifuseCustomBib
   \RequirePackage[square, sort, numbers, authoryear]{natbib} % CustomBib

% If you would like to use biblatex for your reference management, as opposed to the default `natbibpackage` pass the option `custombib` in the document class. Comment out the previous line to make sure you don't load the natbib package. Uncomment the following lines and specify the location of references.bib file

%\RequirePackage[backend=biber, style=numeric-comp, citestyle=numeric, sorting=nty, natbib=true]{biblatex}
%\addbibresource{References/references} %Location of references.bib only for biblatex, Do not omit the .bib extension from the filename.

\fi

% changes the default name `Bibliography` -> `References'
\renewcommand{\bibname}{References}


% ******************************************************************************
% ************************* User Defined Commands ******************************
% ******************************************************************************

% *********** To change the name of Table of Contents / LOF and LOT ************

%\renewcommand{\contentsname}{My Table of Contents}
%\renewcommand{\listfigurename}{My List of Figures}
%\renewcommand{\listtablename}{My List of Tables}


% ********************** TOC depth and numbering depth *************************

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


% ******************************* Nomenclature *********************************

% To change the name of the Nomenclature section, uncomment the following line

\renewcommand{\nomname}{Symbols}

% \makeatletter
% % Main command: if a second argument is provided, define and print full version;
% % if not, print the already-defined short form.
% \newcommand{\acro}[1]{%
%   \@ifnextchar\bgroup{\acro@def{#1}}{\acro@use{#1}}%
% }

% % Definition mode: \acro{<key>}{<definition>}
% \newcommand{\acro@def}[2]{%
%   \ifcsname acro@#1@full\endcsname
%     % If already defined, issue a warning and use the stored version.
%     \PackageWarning{acro}{Acronym `#1' already defined. Using existing definition.}%
%     \acro@use{#1}%
%   \else
%     % Define the full version (for first use) and the short version (for later)
%     \expandafter\def\csname acro@#1@full\endcsname{#2 (\textit{#1})\nomenclature{#1}{#2}}%
%     \expandafter\def\csname acro@#1@short\endcsname{\textit{#1}}%
%     % Mark as already used by setting a flag to 1.
%     \expandafter\def\csname acro@#1@used\endcsname{1}%
%     % Print the full version
%     \csname acro@#1@full\endcsname%
%   \fi
% }

% % Usage mode: \acro{<key>}
% \newcommand{\acro@use}[1]{%
%   \ifcsname acro@#1@full\endcsname
%     % If the acronym was defined, check the “used” flag.
%     \ifnum\csname acro@#1@used\endcsname=1 %
%       % Already used: print short version.
%       \csname acro@#1@short\endcsname%
%     \else
%       % (Fallback: print full version and mark as used.)
%       \expandafter\def\csname acro@#1@used\endcsname{1}%
%       \csname acro@#1@full\endcsname%
%     \fi
%   \else
%     % If no definition exists, issue an error.
%     \PackageError{acro}{Acronym `#1' not defined}%
%       {Define it using \string\acro\string{#1\string}{<definition>} before using it.}%
%   \fi
% }
% \makeatother

\usepackage{xparse}
\makeatletter
\NewDocumentCommand{\acro}{m o}{%
  \IfValueTF{#2}{%
    % Definition mode: if a definition (second argument) is given.
    \ifcsname acro@#1@full\endcsname
      \PackageWarning{acro}{Acronym `#1' already defined. Using existing definition.}%
      \acro@use{#1}%
    \else
      % Save the full version (printed on first use) and short version (for later)
      \expandafter\def\csname acro@#1@full\endcsname{#2 (\textit{#1})\nomenclature{#1}{#2}}%
      \expandafter\def\csname acro@#1@short\endcsname{\textit{#1}}%
      % Mark as used
      \expandafter\def\csname acro@#1@used\endcsname{1}%
      % Print the full version
      \csname acro@#1@full\endcsname%
    \fi
  }{%
    % Usage mode: if no definition is given.
    \ifcsname acro@#1@full\endcsname
      % If already defined, print the short version (if used before)
      \ifnum\csname acro@#1@used\endcsname=1 %
        \csname acro@#1@short\endcsname%
      \else
        % Fallback: print full version and mark as used.
        \expandafter\def\csname acro@#1@used\endcsname{1}%
        \csname acro@#1@full\endcsname%
      \fi
    \else
      \PackageError{acro}{Acronym `#1' not defined}%
        {Define it using \string\acro\string{#1\string}{<definition>} before using it.}%
    \fi
  }%
}
\makeatother



% ********************************* Appendix ***********************************

% The default value of both \appendixtocname and \appendixpagename is `Appendices'. These names can all be changed via:

%\renewcommand{\appendixtocname}{List of appendices}
%\renewcommand{\appendixname}{Appndx}

% *********************** Configure Draft Mode **********************************

% Uncomment to disable figures in `draft'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


% ******************************** Todo Notes **********************************
%% Uncomment the following lines to have todonotes.

%\ifsetDraft
%	\usepackage[colorinlistoftodos]{todonotes}
%	\newcommand{\mynote}[1]{\todo[author=kks32,size=\small,inline,color=green!40]{#1}}
%\else
%	\newcommand{\mynote}[1]{}
%	\newcommand{\listoftodos}{}
%\fi

% Example todo: \mynote{Hey! I have a note}

% ******************************** Highlighting Changes **********************************
%% Uncomment the following lines to be able to highlight text/modifications.
%\ifsetDraft
%  \usepackage{color, soul}
%  \newcommand{\hlc}[2][yellow]{{\sethlcolor{#1} \hl{#2}}}
%  \newcommand{\hlfix}[2]{\texthl{#1}\todo{#2}}
%\else
%  \newcommand{\hlc}[2]{}
%  \newcommand{\hlfix}[2]{}
%\fi

% Example highlight 1: \hlc{Text to be highlighted}
% Example highlight 2: \hlc[green]{Text to be highlighted in green colour}
% Example highlight 3: \hlfix{Original Text}{Fixed Text}

% *****************************************************************************
% ******************* Better enumeration my MB*************
\usepackage{enumitem}

